Near-Optimal Dynamic Rounding of Fractional Matchings in Bipartite Graphs

We study dynamic $(1-\epsilon)$-approximate rounding of fractional matchings -- a key ingredient in numerous breakthroughs in the dynamic graph algorithms literature. Our first contribution is a surprisingly simple deterministic rounding algorithm in bipartite graphs with amortized update time $O(\epsilon^{-1} \log^2 (\epsilon^{-1} \cdot n))$, matching an (unconditional) recourse lower bound of $\Omega(\epsilon^{-1})$ up to logarithmic factors. Moreover, this algorithm's update time improves provided the minimum (non-zero) weight in the fractional matching is lower bounded throughout. Combining this algorithm with novel dynamic \emph{partial rounding} algorithms to increase this minimum weight, we obtain several algorithms that improve this dependence on $n$. For example, we give a high-probability randomized algorithm with $\tilde{O}(\epsilon^{-1}\cdot (\log\log n)^2)$-update time against adaptive adversaries. (We use Soft-Oh notation, $\tilde{O}$, to suppress polylogarithmic factors in the argument, i.e., $\tilde{O}(f)=O(f\cdot \mathrm{poly}(\log f))$.) Using our rounding algorithms, we also round known $(1-\epsilon)$-decremental fractional bipartite matching algorithms with no asymptotic overhead, thus improving on state-of-the-art algorithms for the decremental bipartite matching problem. Further, we provide extensions of our results to general graphs and to maintaining almost-maximal matchings.

==> app-oblivious.tex <==
    
	\section{Addendum: Simple oblivious partial rounding}\label{appendix:oblivious}
	
	One might wonder if our dynamic rounding algorithm's logarithmic dependence on $n$ is necessary. Here we show that for randomized algorithms (against oblivious adversaries), this is not the case: For example, the same approximation ratio can be obtained with only \emph{doubly-logarithmic} dependence on $n$ w.h.p. Moreover, we can 
	replace all occurrences of $L=O(\log(n/\eps))$ by $O(\log(\eps^{-1}))$ in our bounds, thus decreasing the overhead to be a (nearly optimal) constant.
	
	This result is achieved easily, given our deterministic algorithm:
	Randomly sparsify to guarantee that $\min_{e:x_e>0} x_e \geq \eps^2/\log(\eps^{-1})$. This preserves fractional matching values in expectation up to $1-\eps$ loss, with similar results holding for AMFMs (see \cite{arar2018dynamic,wajc2020rounding}).
	Alternatively, guaranteeing that $\x_{\min} = \Omega(\eps^2/\log(n/\eps))$ preserves the matching both in expectation and w.h.p. This decreases $L$ of non-trivial graphs $G_i$ obtained by the fractional matching sampled this way decreases from $\log(\eps^{-1}\cdot n)$ in the deterministic case down to $O(\log(\eps^{-1}))$ or $O(\log\log n + \log(\eps^{-1}))$, respectively.
	This immediately implies the corresponding speedups.
	
	\begin{cor}
	    Let $\eps>0$ and $\alpha=O(1)$. If there exists an $\alpha$-approximate dynamic fractional matching algorithm with update time $T$ and update ratio $C$,
	    then there exist randomized $\alpha(1+\eps)$-approximate dynamic \emph{integral} bipartite matching algorithms with update time $O(T+\eps^{-1}+C\cdot \log^2 (1/\eps)\cdot \eps^{-1})$ and $O(T+\eps^{-1}+C\cdot \log\log(n)\cdot \eps^{-1})$. The algorithms' approximation ratio and update time guarantees hold in expectation and w.h.p., both against an oblivious adversary, respectively.
	\end{cor}
	
	%\section{Minor observation}
	%Given the recent breakthrough maximum flow algorithm, the Gupta/Peng framework in bipartite graphs can be implemented at an $\frac{|E_H|}{\eps \mu}\cdot m^{o(1)}$ cost, where $E_H$ is the sparsifier size. 
	%We maintain a super-sparse sparsifier, of size $O(\mu)$, and avoid having to periodically recompute an approximate (or exact) matching in the sparsifier $H=(V,E_H)$, since this sparsifier is itself a matching. 

==> deamortization.tex <==
\section{Worst-Case Bounds in General Graphs}\label{sec:deamortization}


\begin{thm}
\end{thm}

\begin{lem}

\label{cor:roughcoarsening:worstcase:uniform}

Given dynamic uniform fractional matching $\bf{x}$ and \david{what kind of algorithm?} algorithm $\calA_U$ we can design an alternative variant $\calA_U'$ that has deterministic worst-case update time $O(t_s \cdot \eps^{-1})$ and can be queried to return a fractional matching $\bf{x'}$ in $|\supp{\bf{x'}}|$ time such that $\bf{x'}$ is an $(O(\epsilon + \delta), \delta)$ coarsening of $\bf{x}$.

\end{lem}

\begin{proof}

Let the update sequence of $\bf{x}$ be denoted by $I$. Let $\bf{x_t}$ stand for the state of $\bf{x}$ at time point $t$. Consider a normal run of algorithm $\calA_U$ on $\bf{x}$ under update sequence $I$. Assume that initializations of $\calA_U$ occur at time points $T_0, T_1, \cdots$. Note, that $T_0 = 0$ and $T_i = T_{i-1} + |\supp{\bf{x_{T_{i-1}}}}| \cdot \eps/32$ by definition. $\calA_U'$ will initialize similarly as $\calA_U$. Let $I_i$ stand for the update sequence starting at time point $T_{i-1}$ ending at $T_i$. During each update sequence $I_i$ $\calA_U'$ will calculate an output which will be used as the output when queried during $I_{i+1}$ and forgotten at time $T_{i+1}$. The only exception is at initialization where $\calA_U'$ will simply initialize on $\bf{x_0}$ using $\calA_U$.

For $i \geq 0$ algorithm $\calA_U'$ during the first half of update sequence $I_i$ will calculate the coarsenings $\bf{x^1_{T_{i-1}}}, \dots$ of $\calA_U$ if initialized on $\bf{x_{T_{i-1}}}$. During the second half of $I_i$ $\calA_U'$ deletes any deleted edge in $I_i$ present in any coarsenings $\bf{x^1_{T_{i-1}}}, \dots$. During the processing of the deletions of $I_i$ $\calA_U'$ marks any coarsening with more than $\eps$ fraction of its edges deleted as 'dirty' (but does not discard them from memory as that would not be a worst-case update time operation). If $i=0$ the algorithm does not have to initially administer deletions hence no coarsening is marked dirty. 

We will say that $\calA_U'$ sets its output to be a specific coarsening $\bf{x'}$ during time point $t$ to mean that if $\calA_U$ is queried at time point $t$ it returns $\bf{x'}$ as its solution. Fix some $i$. Between time points $T_i$ and $T_{i+1}$ (that is during $I_{i+1}$) $\calA_U'$ will set its output to be one of the fractional matchings $\bf{x^j_{T_{i-1}}}$ calculated during the processing of the split $I_i$ (or at initialization in case of $i=0$). At time point\sayan{We are using $t$ for update time as well. Better be consistent across the entire paper.} $T_i$ it sets its output to be an arbitrary non-dirty coarsening $\bf{x^j_{T_{i-1}}}$. Throughout the update sequence $I_{i+1}$ whenever a deletion occurs to the support of a coarsening $\bf{x^j_{T_{i-1}}}$ the algorithm updates said coarsening and marks it dirty if an $\eps$ fraction of its edges were deleted. If due to this update the coarsening currently marked as output is marked dirty $\calA_U'$ selects an arbitrary coarsening calculated during $I_i$ yet not marked as dirty to be its output. Note that while this is going on, during the update sequence $I_{i+1}$ $\calA_U'$ is preparing its output coarsenings for the update sub-sequence $I_{i+2}$. The correctness of $\calA_U'$-s output can be shown similarly with larger slack parameters using the analysis of Lemma~\ref{cl:dynamic-coarsening:uniform:rough}.

To argue that $\calA_U'$ has worst-case update time $O(t_s \cdot \eps^{-1})$ first observe that the cost of initializing using $\calA_U$ and $\bf{x_{T_{i-1}}}$ is $O(t_s \cdot |\supp{\bf{x_{T_{i-1}}}}|$. During the first half of $I_i$ this work can be uniformly distributed over $\Omega(\eps \cdot |\supp{\bf{x_{T_{i-1}}}}|)$ updates to receive $O(\eps^{-1} \cdot t_s)$ update time. Administering the deletions of $I_i$ to the coarsenings calculated during the second half of $I_i$ takes $O(I_i)$ time hence can be done in worst-case $O(1)$ time. During update sequences $I_{i+1}$ updating the coarsenings of $I_i$ takes worst-case $O(1)$ time as each update is a single edge deletions. When a coarsening is marked dirty $\calA_U'$ only has to look for an other non-dirty coarsening in its memory. This can be implemented in worst-case $O(1)$ update time through maintaining a set of pointers to non-dirty coarsenings in memory.
\end{proof}

\begin{cor}

\label{cor:roughcoarsening:worstcase}

Given dynamic uniform fractional matching $\bf{x}$ and \david{what kind of algorithm? rounding? coarsening? splitting?...} algorithm $\calA^*$ \david{why star? this only make subsequent notation (star and prime) awkward} we can design an alternative variant ${\calA^*}'$
%\sidford{I added braces to fix a compile bug, might want to check that this is good symbol} 
such that ${\calA^*}'$ has deterministic worst-case update time $O(t_s \cdot \eps^{-1})$ and can be queried to return a fractional matching $\bf{x'}$ in $|\supp{\bf{x'}}|$ time such that $\bf{x'}$ is a rough $(O(\epsilon + \gamma), \delta)$ coarsening of $\bf{x}$.
\end{cor}

\begin{proof}
Follows from  \Cref{lem:split-to-dynamic-coarsening} and \Cref{cor:roughcoarsening:worstcase:uniform}.
\end{proof}


\begin{prop}
\cite{solomon2021generalized}: Assume $\calA$ is a dynamic algorithm with worst-case update time $T$ which can be queried to return an $\alpha$-approximate matching $M$ of graph $G$ in time $|M|$. Using $\calA$ we can design a dynamic algorithm $\calA^*$ which maintains an $\alpha \cdot (1+\eps)$-approximate matching of $G$, has worst-case update time $O(T + \eps^{-1})$ and worst-case recourse $O(\eps^{-1})$.
\end{prop}

\begin{cor}

Assuming $\calR$ has worst-case update time lemma~\ref{lem:dynamic-coarsening-to-rounding} can be modified such that it has worst-case update time and on query returns a solution $M$ in $|M|$ time.

\end{cor}

\begin{proof}

Note that if $\calR$ has worst-case update time then the only computational cost of $\calR^*$ which needs to be amortized comes from the re-initializations (as $\calA^*$ can be implemented with worst-case update time using Corollary~\ref{cor:roughcoarsening:worstcase}). Lets call the worst-case update time variant of $\calR^*$ as ${\calR^*}'$. Define $\bf{x_t}$ to be the state of $\bf{x}$ at time $t$. Let $T_0, T_1 \dots$ stand for the time-points $\calR^*$ re-initializes. Note that $T_0 = 0$ and $T_{i+1}$ only depends on $\norm{\bf{x_{T_{i}}}}$. Let $I_i$ stand for the sequence of updates between $T_{i}$ and $T_{i-1}$. At time $T_0$ ${\calR^*}'$ initializes similarly as $\calR^*$. For any $i \geq 1$ ${\calR^*}'$ completes the following internal computations during the update sequence $I_i$: during the first half of $I_i$ ${\calR^*}'$ uses $\calR^*$ to initialize on fractional matching $\bf{x_{T_{i-1}}}$ and constructs some solution $M_{i-1}$. During the second half of $I_i$ ${\calR^*}'$ uses ${\cal^*}'$ to update $M_{i-1}$ with the updates of $I_i$. Throughout $I_{i+1}$ ${\calR^*}'$ will continue to use $\calR^*$ to update $M_{i-1}$, however it will skip the re-initialization $\calR^*$ would have completed at $T_i$. During $I_{i+1}$ if $\calR^*$ is queried to return a solution it returns the current state of $M_{i-1}$. At the same time during $I_{i+1}$ ${\calR^*}'$ is using $\calR^*$ to prepare $M_i$ which will be used as an answer to queries during $I_{i+2}$ ect.

Focus on the work required to prepare $M_{i-1}$ during sub-sequence $I_i$. The analysis of Lemma~\ref{lem:dynamic-coarsening-to-rounding} that $T_{i}-T_{i-1} = \Omega(\norm{\hat{x_{T_{i-1}}}} \cdot \eps)$ and that re-initializing $\calR^*$ with $\bf{x_{T_{i-1}}}$ takes $O(|\supp{\hat{x_{T_{i-1}}}}|)$ time. Hence, distributing the work of initialization over the first half of $I_i$ we get a worst-case update bound of time of $O(t_I \cdot \eps^{-1})$. In the second half of $I_i$ ${\calR^*}'$ simply needs to make calls to $\calR$ twice as frequently as $\calR^*$ would do to update $M_{i-1}$ with $I_i$.

To argue correctness observe that at time $T_i$ the matching $M_{i-1}$ maintained by ${\calR^*}'$ is the same as the output of $\calR^*$. At this point $\calR^*$ would commence an update as updates to the low value edges $\bf{x_{\leq \delta}}$ could have altered $\norm{\bf{x_{\leq \delta}}}$ by  $\Theta(\eps\cdot \norm{x})$ and $\calR^*$ ignored this updates. However, if $\calR^*$ would have ignored a single re-build, over $I_{i+1}$ $\norm{\bf{x_{\leq \delta}}}$ similarly only changes by at most $\Theta(\bf{x} \cdot \eps)$ hence the effect of these updates on $\bf{x_{\leq \delta}}$ can similarly be ignored until $T_{i+1}$ while only loosing a multiplicative $\epsilon$ factor in approximation. At time ${\calR^*}'$ switched to a new output $M_{i}$ etc.
\end{proof}



==> derandomization.tex <==
\section{Derandomization and Pessimistic  Estimators}

Consider the special case that all low-valued fractions are precisely $1/n$. 
Let $s=1/\Omega(\log n\cdot \eps^{-2})$ be sufficiently small.
We randomly pick one of $ns$ subgraphs to assign each edge to, chosen uniformly and independently, so the probability that $e$ is sampled in subgraph $i\in [ns]$ is precisely $1/(ns)$. Let $X_{i,t}=1$ if the $t^{th}$ edge, $e_t$, is adding to graph $G_i=(V,E_i)$.
A simple application of Chernoff (\Cref{Chernoff}) implies that the maximum degree in each subgraph is at most $(1+\eps)/s$ w.h.p.
Therefore, w.h.p., a fractional matching with value $s/(1+\eps)\geq s(1-\eps)$ per edge in each of these sampled subgraphs is a valid fractional matching (preserving the value up to a $(1-\eps)$ factor).

We now discuss an approach based on the method of conditional probabilities and pessimistic estimators to derandomize the above. For notational simplicity, let us first focus on a single node $v$ and subgraph $G_i$, and drop the relevant indices.

The proof of \Cref{Chernoff} yields a pessimistic estimator for the probability that a vertex overshoots its expected degree, specifically, if $X=\sum_k X_k$ for independent $X_k\in [0,1]$, then 
\begin{align*}
\Pr[X\geq (1+\eps)\E[X]] & \leq \Pr[\exp(X)\geq \exp((1+\eps)\E[X])] \\
& \leq \frac{\E[(1+\eps)^X]}{(1+\eps)^{(1+\eps)\E[X}]} \\
& \leq \frac{\prod_k \E[(1+\eps)^{X_i}]}{(1+\eps)^{(1+\eps)\E[X]}} \\
& \leq \frac{\prod_k \E[1+\eps\cdot X_i]}{(1+\eps)^{(1+\eps)\E[X]}},
\end{align*}
where the last inequality relies on convexity and $(1+\eps)^z\leq 1+\eps z$ if $z\in [0,1]$.
Further algebraic manipulations result in polynomial tail bounds if $\E[X]=\Omega(\log n \cdot \eps^{-2})$, as is the case in our applications of the Chernoff bound.
Now, denoting the RHS of the above by $\phi := \frac{\prod_i \E[1+\eps\cdot X_i]}{(1+\eps)^({1+\eps)}}$, the values obtained by partial derandomization of the r.v.s $X_1,\dots,X_t$ (conditioning) is given by 
\begin{align*}
\E[\phi \mid X_1=x_1,\dots,X_t=x_t] = \frac{\prod_{k=t+1}^n \E[1+\eps\cdot X_k]}{(1+\eps)^{(1+\eps)\E[X]}} \times \prod_{k=1}^t \E[1+\eps\cdot x_k]. 
\end{align*}
We will let the RHS after setting $t=0,1,\dots$ many r.v.s, denoted by $\Psi_0,\Psi_1,\dots$, serve as our pessimistic estimator for the event that $X\geq (1+\eps)\E[X]$.
By linearity of expectation, there exists some assignment of $X_t\gets x_t$ that guarantees $\Psi_t\leq \Psi_{t-1}$.
For the above simple case of a single Chernoff bound, we have specifically that 
\begin{align}\label{chernoff-pessistic-estimator-change}
\Psi_t = \frac{1+\eps \cdot x_t}{1+\eps \cdot \E[X_t]}\times \Psi_{t-1}.
\end{align}
Proceeding in this fashion we obtain an assignment $\vec{X}\gets \vec{x}$ with $\Psi_n \leq \Psi_0 < 1$, and so the final assignment (deterministically) satisfies $X\leq (1+\eps)\E[X]$.

In our problem, we wish to derandomize a number of Chernoff bounds combined with a union bound.
We can therefore consider the sum of the above pessimistic estimators. By union bound, we have that the sum of these estimators (upper bounding the probability of some vertex having its degree be greater than $1/s=\Omega(\log n \cdot \eps^{-2})$ in some subgraph $G_i$ is polynomially small, and so if the sum of the above $\Psi_t$ (for each vertex and each subgraph) is non-increasing in $t$, we obtain that the final assignment of edges to subgraphs results in subgraphs $G_i=(V,E_i)$ in which the uniform fractional matching $\frac{s}{1+\eps}\cdot \mathbf{1}^{E_i}$ is a feasible fractional matching.

\paragraph{The challenge.} 
While it is clear that for each edge $e\in E$, one can find some $i$ such that adding $e$ to $E_i$ does not increase the pessimistic estimator, it is not immediately clear how to find this index $i$.
For every vertex $v$ and subgraph $i$, let $\Psi^{v,i}_t$ be the pessimistic estimator for the upper Chernoff bound given above.
Then, \Cref{chernoff-pessistic-estimator-change} gives us a closed form for the effect of assigning $e_t$ to $E_i$:
\begin{align*}
\Psi^{w,j}_t = \begin{cases} \frac{1+\eps}{1+\eps / (n\cdot s)}\times \Psi^{w,j}_{t-1} & w\in e,\,\textrm{ and } j=i \\
\frac{1}{1+\eps / (n\cdot s)}\times \Psi^{w,j}_{t-1} & w\in e,\,\textrm{ and } j\neq i \\
\Psi^{w,j}_{t-1} & \textrm{else.}
\end{cases}
\end{align*}
So, by induction, we have that $$\Psi^{v,i}_t = \frac{(1+\eps)^{d_{i,t}(v)}}{(1+\eps/ (n\cdot s))^{|\delta(v)\cap \{e_1,\dots,e_t\}|}}\times \Psi^{v,i}_0,$$ 
where $d_{i,t}(v) := \sum_{t: e_t\ni v} X_{i,t}$ is the number of edges in $\delta(v)\cap E_i \cap \{e_1,\dots,e_t\}$, i.e., the number of edges of $v$ added to $E_i$ among the first $t$ edges in $E$.

\color{red}
For each $t=1,\dots,m$, the existence of some choice of $E_i$ to add $e_t$ to while decreasing $\Phi_t:=\sum_{v,j,t} \Psi^{v,j}_t$ (compared to $\Phi_{t-1}$) is immediate by linearity of expectation, but finding this $i$ in constant or near-constant amortized time per edge is less apparent.\david{at least to me right now}
\color{black}

\paragraph{Plausible approach?}
Recall that we start with $\Phi_0 \leq 1/\poly(n)$. 
We can therefore slightly deviate from the method of conditional expectations and not guarantee that $\Phi_t\leq \Phi_{t-1}$, but instead just guarantee that over the $m=\poly(n)$ setting of variables, we only increase $\Phi_t$ by a small polynomial multiplicative factor compared to $\Phi_0$.
For example, we can afford to have for each time $t$ that $\Phi_t\leq (1+\frac{O(\log n)}{m})\cdot \Phi_{t-1}$, resulting in $\Phi_m \leq (1+\frac{O(\log n)}{m})^m\cdot \Phi_0 \leq \poly(n)/\poly(n) < 1$, and so this too will result in a good partitioning.



\paragraph{Useful data structures?}
We note that, if we manage to guarantee that $d_{i,t}(v)\leq O(\log n\cdot \eps^{-2})$ for each triple $(i,t,v)$, then we can maintain for each vertex $v$ a BST/priority queue for indices $i$ with priority $d_{i,t}(v)$, with all operations taking only $\poly(\log\log n,\, \log(1/\eps))$ time.\footnote{In fact, if all we need is the ability to increment $d_{i,t}(v)$ and extract a min/max, then since $d_{i,t}(v)$
is a monotonically increasing integer, increasing by one whenever it increases, 
we can easily support both operations in constant time using nothing more than arrays and lists.
} 

\paragraph{Choosing $i$}
Consider an edge $e_t=(u,v)$.
\color{red}Question/Problem: \color{black} What data structures allow to quickly find an index $i$ such that $(1+\eps)^{d_{i,t}(u)}/(1+\eps/ (n\cdot s))^{|\delta(u)\cap \{e_1,\dots,e_{t-1}\}|}$ summed with its counterpart for $v$ are small? (Approximately minimal?)

\subsection{Scratch paper}

Maximum ratio between contributions to $\Phi$ for different nodes in the same subgraph, assuming $d_{i,t}\leq O(\log n \cdot \eps^{-2})$, is at most
$(1+\eps)^{O(\log n \cdot \eps^{-2})} \leq \exp(O(\log n \cdot \eps^{-1})) = n^{O(\eps^{-1})}$. 

Increase by factor $(1+\eps/2)$ by penalizing only one of the two.
However, $(1+\eps/2)^m\leq \exp(\eps\cdot m/2)$.


Say use $s=1/\Omega(\log n \cdot \eps^{-r})$ and manage to guarantee $d_{i,t}(v)\leq 1/s$ for each triple $(i,t,v)$.
Then, ratio of values is at most 
\begin{align*}
(1+\eps)^{O(\log n \cdot \eps^{-r})} = O(n^{\eps^{-r+1}}).
\end{align*}
On the other hand, 
\begin{align*}
\Pr[X\geq (1+\eps)\cdot \E[X]] \leq \exp\left(-\frac{\eps^2\cdot \E[X]}{3}\right) = O(n^{-\eps^{-r+2}}).
\end{align*}
